Parametric Interval Temporal Logic over Infinite Words

Model checking for Halpern and Shoham's interval temporal logic HS has been recently investigated in a systematic way, and it is known to be decidable under three distinct semantics. Here, we focus on the trace-based semantics, where the infinite execution paths (traces) of the given (finite) Kripke structure are the main semantic entities. In this setting, each finite infix of a trace is interpreted as an interval, and a proposition holds over an interval if and only if it holds over each component state (homogeneity assumption). In this paper, we introduce a quantitative extension of HS over traces, called parametric HS (PHS). The novel logic allows to express parametric timing constraints on the duration (length) of the intervals. We show that checking the existence of a parameter valuation for which a Kripke structure satisfies a PHS formula (model checking), or a PHS formula admits a trace as a model under the homogeneity assumption (satisfiability) is decidable. Moreover, we identify a fragment of PHS which subsumes parametric LTL and for which model checking and satisfiability are shown to be EXPSPACE-complete.

==> Abstract.tex <==

The model-checking (MC) problem of Halpern and Shoham Interval Temporal Logic (\HS) has been recently investigated in some papers and is known to be decidable. An intriguing open question concerns the exact complexity of the problem for full $\HS$: it is at least $\EXPSPACE$-hard, while
 the only known upper bound is  non-elementary and is obtained by exploiting an abstract representation of Kripke structure paths called \emph{descriptors}.
In this paper we generalize the approach by providing a uniform framework for model-checking full $\HS$ and meaningful (almost maximal) fragments,
where a specialized type of descriptor is defined for each fragment. We then devise a general MC alternating algorithm
parameterized by the type of descriptor which has  a polynomially bounded number of alternations and whose running time is bounded
by the length of minimal representatives of descriptors (certificates). We analyze the time complexity of the algorithm and give, by non-trivial arguments,
tight bounds on the length of certificates. For two types of descriptors, we obtain exponential upper and lower bounds which lead to an elementary MC algorithm
for the related $\HS$ fragments. For the other types of descriptors, we provide non-elementary lower bounds. This last result
addresses a question left open in some papers regarding the possibility of fixing an elementary upper bound on the size of  the descriptors for full $\HS$.

%We study open complexity issues of the model checking problem for the Halpern - Shoahn Interval Temporal Logic (\HS). The decidability of the problem for  \HS\ has been proved by a non elementary procedure exploiting an abstract representation of Kripke structure paths called \emph{descriptors}.
% devising a general model checking procedure which can be applied to the full logic and meaningful fragments fixing tight complexity bounds. Moreover, the best known lower bound places the model checking problem of the full logic in $\EXPSPACE$ and any attempt to find a matching lower bound has been in this years unfruitful. An insight to that hard open problem is given by the non-elementary succinctess of \emph{descriptors} proved in the paper which shows  that, if elementary model checking procedures are possible, they have certaintly to exploit less powerful structures. lower bound places the model checking problem of the full logic in $\EXPSPACE$ and any attempt to find a matching lower bound has been in this years unfruitful. An insight to that hard open problem is given by the non-elementary succinctess of \emph{descriptors} proved in the paper which shows  that, if elementary model checking procedures are possible, they have certaintly to exploit less powerful structures. 

==> eptcsdata.tex <==
\providecommand{\firstpage}{97}
\providecommand{\publicationstatus}{D. Della Monica and P. Ganty (Eds.): 13th International Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF 22)\\
EPTCS 370, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.370.7}{10.4204/EPTCS.370.7}}

